Optimizing the Long-Term Behaviour of Deep Reinforcement Learning for Pushing and Grasping

We investigate the "Visual Pushing for Grasping" (VPG) system by Zeng et al. and the "Hourglass" system by Ewerton et al., an evolution of the former. The focus of our work is the investigation of the capabilities of both systems to learn long-term rewards and policies. Zeng et al. original task only needs a limited amount of foresight. Ewerton et al. attain their best performance using an agent which only takes the most immediate action under consideration. We are interested in the ability of their models and training algorithms to accurately predict long-term Q-Values. To evaluate this ability, we design a new bin sorting task and reward function. Our task requires agents to accurately estimate future rewards and therefore use high discount factors in their Q-Value calculation. We investigate the behaviour of an adaptation of the VPG training algorithm on our task. We show that this adaptation can not accurately predict the required long-term action sequences. In addition to the limitations identified by Ewerton et al., it suffers from the known Deep Q-Learning problem of overestimated Q-Values. In an effort to solve our task, we turn to the Hourglass models and combine them with the Double Q-Learning approach. We show that this approach enables the models to accurately predict long-term action sequences when trained with large discount factors. Our results show that the Double Q-Learning technique is essential for training with very high discount factors, as the models Q-Value predictions diverge otherwise. We also experiment with different approaches for discount factor scheduling, loss calculation and exploration procedures. Our results show that the latter factors do not visibly influence the model's performance for our task.

==> main/acknowledgements.tex <==
% !TeX spellcheck = en_US
% !TeX encoding = UTF-8
% !TeX root = ../thesis.tex

\chapter*{Acknowledgements}
\addcontentsline{toc}{chapter}{Acknowledgements}

I would like to thank my advisors, \advisor and \advisortwo, as well as \referee, for their great input and advice. I would also like to thank Marco Ewerton, Angel Martínez-González and Jean-Marc Odobez from the Idiap Research Institute for sharing their pre-published work and Maximillian Li for his support in any questions regarding the ALR simulation framework.

I would also like to thank my family and friends for their love and support.

The authors acknowledge support by the state of Baden-Württemberg through bwHPC.

==> template/alr_def.tex <==
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %
% ARL Paper Definitions
%
% Please include this file in all ALR papers and use the definitions
% as a common standard.
%
% If something is missing in this file, please extend it, but keep
% it simple and don't pollute it.
%
% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

% Packages
\usepackage[per-mode=fraction]{siunitx}
\usepackage{comment}
\usepackage[normalem]{ulem}
\usepackage{xspace}

% Units commonly used in robotics
\DeclareSIUnit\px{px}
\DeclareSIUnit\fps{fps}

% Colors
\definecolor{OliveGreen}{RGB}{0,200,25}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\darkgreen}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}

% Abbreviations
\newcommand{\ie}{i.\,e.\, }
\newcommand{\eg}{e.\,g.\, }
\newcommand{\etal}{et\,al.\ }

% Revision macros
\newcommand{\added}[1]{\darkgreen{#1}}
\newcommand{\replaced}[2]{\red{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}\darkgreen{#2}}
\newcommand{\removed}[1]{\red{\ifmmode\text{\sout{\ensuremath{#1}}}\else\sout{#1}\fi}}
\newcommand{\remark}[1]{\blue{#1}}

% Uncomment the following lines for the final version (without revision marks)
% Attention: Always check the final version!
%            Misplaced revision macros might add unwanted spaces.

\begin{comment}
	\renewcommand{\added}[1]{#1}
	\renewcommand{\replaced}[2]{#2}
	\renewcommand{\removed}[1]{}
\end{comment}

% More complex revision macros (for rebuttal letters, subject to extension)
\newcommand{\addedimage}[1]{\fcolorbox{blue}{blue}{#1}}
\newcommand{\removedfootnote}[1]{\footnote{\removed{#1}}}
\newcommand{\removedsubsection}[1]{\subsection{\texorpdfstring{\removed{#1}}{#1}}}
\newcommand{\replacedsubsection}[2]{\subsection{\texorpdfstring{\removed{#1}\added{#2}}{#2}}}
\newcommand{\addedsection}[1]{\section{\texorpdfstring{\added{#1}}{#1}}}

% Uncomment the following lines for the final version (without revision marks)
% Attention: Always check the final version!
\begin{comment}
	\renewcommand{\addedimage}[1]{#1}
	\renewcommand{\removedfootnote}[1]{}
	\renewcommand{\removedsubsection}[1]{}
	\renewcommand{\replacedsubsection}[2]{\subsection{#2}}
	\renewcommand{\removedsubsection}[1]{}
\end{comment}


